Adaptive Multiple-Arm Identification

We study the problem of selecting $K$ arms with the highest expected rewards in a stochastic $n$-armed bandit game. This problem has a wide range of applications, e.g., A/B testing, crowdsourcing, simulation optimization. Our goal is to develop a PAC algorithm, which, with probability at least $1-\delta$, identifies a set of $K$ arms with the aggregate regret at most $\epsilon$. The notion of aggregate regret for multiple-arm identification was first introduced in \cite{Zhou:14} , which is defined as the difference of the averaged expected rewards between the selected set of arms and the best $K$ arms. In contrast to \cite{Zhou:14} that only provides instance-independent sample complexity, we introduce a new hardness parameter for characterizing the difficulty of any given instance. We further develop two algorithms and establish the corresponding sample complexity in terms of this hardness parameter. The derived sample complexity can be significantly smaller than state-of-the-art results for a large class of instances and matches the instance-independent lower bound upto a $\log(\epsilon^{-1})$ factor in the worst case. We also prove a lower bound result showing that the extra $\log(\epsilon^{-1})$ is necessary for instance-dependent algorithms using the introduced hardness parameter.

==> preliminary.tex <==
\section{Preliminaries}

\xnote{Maybe put this to the appendix?}
% \begin{lemma}[Chernoff Bound]
%   \label{lem:chernoff}
% Let $X_1, \ldots, X_n$ be independent random variables where $X_i \in [0,1]$. Let $X = X_1 + \ldots + X_n$.  For any $\eps \geq 0$, we have
%   $$\Pr[X \geq (1 + \eps)\bE[X]] \leq \exp\left(- \frac{\eps^2 \bE[X]}{3}\right) \ \ \text{and} \ \  \Pr[X \leq (1 - \eps)\bE[X]] \leq \exp\left(-\frac{\eps^2\bE[X]}{2} \right).$$
% \end{lemma}


\begin{lemma}[Hoeffding's Inequality]
  \label{lem:bound-dist}
  Let $\mathcal{D}$ be a distribution with a bounded support $[0, 1]$, Let $X_1, \ldots, X_n \iid \mathcal{D}$, and $X = \frac{1}{n}\sum_{i=1}^nX_i$. For any $\eps > 0$, we have
  $$\Pr[X \geq \bE[X] + \eps] \leq \exp\left(-2n\eps^2\right)
  \text{and} \ \
  \Pr[X \leq \bE[X] - \eps] \leq \exp\left(-2n\eps^2\right).$$
\end{lemma}
%\xnote{It seems to me that this Hoeffding's statement is wrong.  It should be $\Pr[X \geq \bE[X] + \eps] \leq \exp\left(-2n\eps^2\right)$. Please check!}
%\qinsays{this is from Jiecao, but I don't think it matters: $\exp\left(-\frac{n\eps^2}{2}\right)$ is also okay}
\ynote{I don't think we need formally state Hoeffding's inequality.}

\begin{lemma}
  \label{lem:delta-order}
Given $\mu_1 \geq \ldots \geq \mu_n$ and $\Delta > 0$, assuming that $|\tmu_i - \mu_i| \leq \Delta$ for all $i \in [n]$, and letting $y_1 \geq \ldots \geq y_n$ be the sorted version of $\tmu_1, \ldots, \tmu_n$, we have $|y_i - \mu_i| \leq \Delta~~\text{for all}~ i \in [n]$.
\end{lemma}
\ynote{Consider moving this into the proof.}


%\paragraph{Problem Definition}
%In the {\bf \arm} problem we have $n$ arms, each following an unknown distribution with support $[0,1]$. W.l.o.g., we assume $\theta_1 \geq  \dots \geq \theta_n$ where each $\theta_i$ is the expectation of the distribution (or the {\em true-mean}) of the $i$-th arm. The indices of the arms are unknown in advance. Our goal is to select by pulling the arms a set $T \subseteq [n]$ of $K$ arms so that
%\begin{eqnarray}\label{eq:regret}
%\frac{1}{K} \left( \sum_{i \in T} \theta_i  - \sum_{i \in [K]} \theta_i \right) \leq \eps.
%\end{eqnarray}
%We refer arms in $T$ as \textbf{\arm}. Note that such $T$ may not be unique.
%
%\xnote{Just confirm that the R.V. just needs to be supported on $[0,1]$? Our previous paper assumes the R.V. is binary.}



%\xnote{Why $H^{(0, t)} = \Omega(n/\epsilon)$ ?}



